On early and late phases of acceleration of the expansion of the universe

This thesis tackles the vast question of generating accelerated periods of expansion of the universe. Models loosely related were developed in the early and late universe. In the early universe, generalizations of the Schwinger effect were developed in curved (de Sitter) space and some backreaction effects were estimated. In the late universe, a fractal model was developed and confronted to supernovae data. This relies on the idea of an accelerated expanding universe being nothing but a mirage due to inhomogeneities disposed in a fractal (in this particular model) way. Finally a model of interacting energy based on an Einstein-Cartan gravitational theory was phenomenologically investigated.

==> cours/L2.tex <==
\paragraph{}We just previously discuss that the modern cosmology is based on two pillars: \textit{the cosmological principle} and the assumption that we can describe the whole Universe with\textit{ general relativity}. General relativity is a theory which is willing to explain all gravitational processes with 10 non-linear, coupled differential field equations. These equations relate the geometry of the Universe to the energy content of it. To hope solving these equations, one have to assume symmetry of the space-time (ie. the geometry) and of the matter distribution, this is formlized with the cosmological principle.
\paragraph{} We will go now through some aspects of the formalism of GR and then apply it to our Universe. To do this, we will simplify the Einstein equations with the help of the cosmological principle. We hope that we will eventually recover the Hubble law which was empirical before. Furthermore, from 10 field equations, we will simply have 2 independant equations that we have seen in the previous lecture: the Friedmann equations.
\section{Notions of differential geometry}
As an introduction let us consider special relativity in cartesian coordinates. The world line element can be written:
\begin{equation}
\mathrm{ds}^{2}= \mathrm{ dt}^{2}-\mathrm{dx}^{2}-\mathrm{dy}^{2}-\mathrm{dz}^{2}=\eta_{\mu \nu}\mathrm{dx}^{\mu}\mathrm{dx}^{\nu}=\vec{\mathrm{dx}} \hspace{0.1cm}\mathrm{\eta}\hspace{0.1cm} \vec{\mathrm{dx}}
\end{equation}\\
We introduce now $\tau$ such that: $\mathrm{ds}^{2}=\mathrm{d\tau}^{2}$. It is called the proper time.\\
$\eta$ is the metric tensor of the 4-dimensional Minkowski space-time. $\eta_{\mu \nu}$ are the components of $\eta$. In the most general case, the number of independent components is 10 (as for every 4 by 4 symmetric matrix). In our case it is 4 (x,y,z,t). From now, we will be less precise with the difference between tensor and component of the tensor. For instance, we will say that in cartesian coordinates, $\eta_{\mu \nu}= \mathrm{diag}(1,-1,-1,-1)$.
\subsection{Positive definite metric (=space)}
\paragraph{Flat space}
In this paragraph, we will focus on the spatial part of the metric. Let us rewrite: 
\begin{equation}
\mathrm{ds}^{2}= \mathrm{ dt}^{2}-\mathrm{dx}^{2}-\mathrm{dy}^{2}-\mathrm{dz}^{2}=\mathrm{dt}^{2}-\mathrm{h}_{\mathrm{i j}}\mathrm{dx}^{i}\mathrm{dx}^{j}
\end{equation}\\
$h_{ij}$ are the components of the 3D homogeneous, isotropic, euclidian space. In spherical coordinates, one can also write this metric: 
\begin{equation}
\mathrm{ds}^{2}= -\mathrm{ dt}^{2}+\mathrm{dr}^{2}+r^{2}(\mathrm{d}\theta^{2}+\sin^{2} \theta \hspace{0.1cm}\mathrm{d}\phi^{2})
\end{equation}
\paragraph{Curved space}
There exists also curved\footnote{To begin, we will only focus on positively curved spaces.} spaces: for instance the surface of a sphere is a 2d positively curved space. We call it sometimes a 2-Sphere (or S2). Let us consider this 2d sphere as embedded\footnote{One can always embed positively curved n-dimentianal space  in n+1 euclidian space and n negatively curved space in n+2 minkowskian space.} in our usual 3d euclidian space. The equation for this sphere of radius R is $x^{2}+y^{2}+z^{2}=R^{2}$ which gives by differentiating $\text{d}z=-\frac{x\text{d}x+y\text{d}y}{\sqrt{R^{2}-\text{d}x^{2}-\text{d}y^{2}}}$. Hence we can deduce the line element for the sphere embedded in the 3-d euclidian space: $\mathrm{ds}^{2}= \mathrm{ dx}^{2}+\mathrm{dy}^{2}+\mathrm{dz}^{2}=\mathrm{ dx}^{2}+\mathrm{dy}^{2}+\frac{(x\text{d}x+y\text{d}y)^{2}}{R^{2}-x^{2}-y^{2}}$. We can remark that there is a south-north degeneracy. The independant coordinates x and y vary in $\mathbb{R}$ with the condition $x^{2}+y^{2}<R^{2}$. We see that the equator (z=0) is not described by this set of coordinate. By setting for convenience: x= r' cos$\varphi$ and y= r' sin$\varphi$, we get: 
\begin{equation}
\text{dl}^{2}= \frac{\text{dr'}}{1-\left(\frac{r'}{R}\right)^{2}}+r'^{2} d\varphi^{2}
\end{equation}
There is a bunch of remarks one can do about this formula. If we set $R=\infty$, we recover the 2D flat space. Furthermore if we assume $R^{2}<0$, we get an hyperbolic\footnote{Lobachewski space} 2D space. The metric can be writen in this case: $\text{dl}^{2}= \frac{\text{dr'}}{1+\left(\frac{r'}{R}\right)^{2}}+r'^{2} d\varphi^{2}$.
\paragraph{Rescaling} A simple rescaling $\left( r=\frac{r'}{\sqrt{|R|^{2}}}\right)$ gives $\text{dl}^{2}= |R|^{2}\left(\frac{\text{dr}}{1-kr^{2}}+r^{2} d\varphi^{2}\right)$, where k=$\pm1$ or 0 denotes is the curvature is respectively positive, negative or null. $R^{2}$ is the square of the radius of curvature.
\paragraph{Back to a more familiar form} Let's substitute d$\theta^{2}=\frac{\text{dr}}{1-kr^{2}}+r^{2}d\varphi^{2}$, we get 
\begin{align}
r=f_{k}(\theta)=  \sin(\theta), & k=+1 \\
 \theta, & k=0, \\
 \sinh(\theta), & k=-1
\end{align} 
and the metric takes the following form:
\begin{equation}
\text{dl}^{2}=R^{2}\left(d\theta^{2}+f_{k}^{2}(\theta)\text{d}\varphi^{2}\right)
\end{equation}
\underline{Rem:} This can be generalised to n dimensions and the 3D case will be useful later: $\text{dl}^{2}=R^{2}\left(d\chi^{2}+f_{k}^{2}\left(\text{d}\theta^{2} + \sin^{2}(\theta)\text{d}\varphi^{2}\right)\right)$
\paragraph{More fun with 3D hyperspaces:} Let us consider all the points lying at fixed $\chi$ in the 3D case presented before. The object we are considering is simply a 2-sphere of radius\footnote{This is not precisely a radius in the common sense we are used to, since $\chi$ is dimensionless. Nevertheless one can think of the generalisation to curved spaces to the radius. The analogy is not to be taken too far as we will see in this paragraph.} $\chi$. We get for the line element:
\begin{equation}
dl^{2}=R^{2}f_{k}^{2}(\chi)\left(\text{d}\theta^{2} + \sin^{2}(\theta)\text{d}\varphi^{2}\right),
\end{equation}  which is identical to the line element on a 2-sphere of radius R with an extra factor $f_{k}^{2}(\chi)$. The total surface is then:
\begin{equation}
S=4 \pi R^{2} f_{k}^{2}(\chi)
\end{equation}
There are various interesting facts about this formula:\\
$\bullet$ For k=0, we recover the ordinary result. \\
$\bullet$ For k=-1, $f_{k}^{2}(\chi)=\sinh \chi$ and for $\chi = \infty$, $S=\infty$. \\
$\bullet$ For k=1, $f_{k}^{2}(\chi)=\sin \chi$, with $\chi \in [0,\pi]$ and hence there is two values for which the surface is zero ($\chi=0,\pi$) and one value of $\chi=\frac{\pi}{2}$ for which the surface is maximal.
\paragraph{What about the volume?}
Defining $V \equiv \int_{0}^{\chi} S \text{dl}$, we get $V=\textcolor{red}{\textbf{TBC}}$. We se that $V_{k=1}(\chi=\pi)=2\pi^{2}R^{3}$ which is finite whereas the surface was zero. $V_{k=0}$ and $V_{k=1}$ go to infinity for $\chi = \infty$.
\paragraph{} As said before, the metric we are considering is relevant in cosmology since it describes the spatial slices of our Universe. We then understand that the questions about the values of the surface and the volume of our Universe can be confusing for these curved spaces and the answers can be quite different from the flat case and so are to be taken with great care. Today, most of the cosmologists believe that the space is flat (k=0), hence the volume of our Universe would be infinite. A last world on this last statement; our current understanding of our Universe on both theoretical and observational state is for a flate infinite Universe but nobody what the future development will be like and maybe we will find out new exotic geometry for It in the next years. For instance,the question of the volume of the Universe which is related to the topology of the Universe which can be non trivial and hence can lead to finite volume.
\subsection{What about time?}
We considered in the previous paragraph only space and not space-time. We will discuss it a bit and derive the geodesic equation in 2D which governs the movment of the free falling observers in GR. Let us consider the cartesian coordinates  $x^{i}=(x,y)$. The equation of motion is then $\frac{d^{2}x^{i}}{dt^{2}}=0$.  Let us consider a general change of coordinate (eg. move to $\tilde{x}=(r,\theta)$). We have $x^{i}=x^{i}(\tilde{x^{j}})$ and hence by differentiating, we get $\frac{dx^{i}}{dt}=\frac{\partial x^{i}}{\partial \tilde{x^{j}}} \frac{d \tilde{x^{j}}}{dt}$, where $\frac{\partial x^{i}}{\partial \tilde{x^{j}}}$ is the jacobian matrix of the transformation. We then have: 
\begin{eqnarray*}
\frac{\text{d}^{2}x^{i}}{\text{dt}^{2}}&=& \frac{\text{d}}{\text{dt}}\left( \frac{\partial x^{i}}{\partial \tilde{x^{j}}} \frac{\text{d} \tilde{x^{j}}}{\text{dt}} \right)=0 \text{ (Newton second law}) \\
&=&  \frac{\text{d}}{\text{dt}}\left( \frac{\partial x^{i}}{\partial \tilde{x^{j}}}\right)\frac{\text{d} \tilde{x^{j}}}{\text{dt}}+\frac{\partial x^{i}}{\partial \tilde{x^{j}}}\frac{\text{d}^{2}\tilde{x}^{j}}{\text{dt}^{2}} \\
\end{eqnarray*}
Using the fact that $\frac{\text{d}}{\text{dt}}\left( \frac{\partial x^{i}}{\partial \tilde{x^{j}}}\right)=\frac{\partial}{\partial \tilde{x}^{j}}\left(\frac{dx^{i}}{dt}\right)=\frac{\partial}{\partial \tilde{x}^{j}}\left(\frac{\partial x^{i}}{\partial \tilde{x^{k}}}\right)=\frac{\partial^{2}x^{i}}{\partial \tilde{x}^{j}\partial \tilde{x}^{k}} \frac{\text{d} \tilde{x^{k}}}{\text{dt}}$, multiplying by the inverse jacobian matrix and setting $\Gamma _{\text{jk}}^{l} \equiv \frac{\partial^{2}x^{i}}{\partial \tilde{x}^{j}\partial \tilde{x}^{k}} \frac{\partial x^{l}}{\partial \tilde{x}^{i}}$, we get the so-called geodesic equation:
\begin{equation}
\ddot{x}^{l}+\Gamma_{\text{jk}}^{l}\dot{x}^{k}\dot{x}^{j}=0
\end{equation}
The dot denotes the derivative with respect to t. One of GR founding principles is the equivalence principle which states that there exists, for massive particles, freely falling coordinate systems (inertial) in which the acceleration is given by $\frac{d^{2}y^{\mu}}{d\tau^{2}}=0$. $\tau$ is the proper time which is defined for massive particles. The link with the geodesic equation is that the Christophel symbols can locally vanish in a well-suited\footnote{The Christophel symbols involve only first derivates of the metric and the gravitational effects are present in the second derivative of it (tidal force), that is why one can always remove them. The Christophel symbols represent how non-inertial a given set of coordinate is.} set of coordinate. Since Christophel symbols are not tensors, this does not imply they vanish in every set of coordinate.
We will now move to the application of this formalism to cosmology.
\section{Apply this new tools to cosmological purpose}

